Non-adaptive probabilistic group testing with noisy measurements: Near-optimal bounds with efficient algorithms

We consider the problem of detecting a small subset of defective items from a large set via non-adaptive "random pooling" group tests. We consider both the case when the measurements are noiseless, and the case when the measurements are noisy (the outcome of each group test may be independently faulty with probability q). Order-optimal results for these scenarios are known in the literature. We give information-theoretic lower bounds on the query complexity of these problems, and provide corresponding computationally efficient algorithms that match the lower bounds up to a constant factor. To the best of our knowledge this work is the first to explicitly estimate such a constant that characterizes the gap between the upper and lower bounds for these problems.

==> analysisCBP_tmp.tex <==
\noindent {\bf Proof of Theorem~\ref{thm:3}}:

The Coupon Collector's Problem (CCP) is a classical problem that considers the following scenario. Suppose there are $n$ types of coupons, each of which is equiprobable. A collector selects coupons (with replacement) until he has a coupon of each type. What is the distribution on his stopping time? It is well-known (\cite{wiki:ccp}) that the expected stopping time is $n\ln n + \Theta(n)$. Also, reasonable bounds on the tail of the distribution are also known -- for instance, it is known that the probability that the stopping time is more than $\chi n \ln n$ is at most $n^{-\chi + 1}$.

%Analogously to the above, we view the group-testing procedure of CBP as a Coupon Collector Problem. Consider the following thought experiment. Suppose we consider any test as a length-$g$ {\it test-vector } \footnote{Note that this test-vector is different from the binary length-$n$ vectors that specify tests in the group testing-matrix, though there is indeed a natural bijection between them.} whose entries index the items being tested in that test (in this view, repeated entries are allowed in this vector). Due to the design of our group testing procedure in CBP, the probability that any item occurs in any location of such a vector is uniform and independent. In fact this property (uniformity and independence of the value of each entry of each test) also holds {\it across} tests. Hence, the items in any subsequence of $k$ tests may be viewed as the outcome of a process of selecting a single chain of $gk$ coupons. This is still true even if we restrict ourselves solely to the tests that have a negative outcome.
%The goal of CBP may now be viewed as the task of collecting {\it all} the {\it negative} items. This can be summarized in the following equation.

Analogously to the above, we view the group-testing procedure of CBP as a Coupon Collector Problem. Consider the following thought experiment. Suppose we consider any test as a length-$g$ {\it test-vector } \footnote{Note that this test-vector is different from the binary length-$n$ vectors that specify tests in the group testing-matrix, though there is indeed a natural bijection between them.} whose entries index the items being tested in that test (in this view, repeated entries are allowed in this vector). Due to the design of our group-testing procedure in
CBP, the probability that any item occurs in any location of such a vector is uniform and independent. In fact this property (uniformity and independence of the value of each entry of each test) also holds {\it across} tests. Hence, the items in any subsequence of $k$ tests may be viewed as the outcome of a process of selecting a single chain of $gk$ coupons. This is still true even if we restrict ourselves solely to the tests that have a negative outcome. The goal of CBP may now be viewed as the task of collecting {\it all} the {\it negative} items. This can be summarized in the following equation

\begin{equation}
\label{eq:1}
Tg\left ( \frac{n-d}{n} \right )^g \geq (n-d)\ln (n-d) .
\end{equation}

Modifying (\ref{eq:1}) to obtain the corresponding tail bound on $T$ takes a bit more work. The right-hand side is then modified to $\chi (n-d) \ln (n-d)$ (which corresponds to the probability that all types of coupons have not been collected if these many total coupons have been collected is at most $(n-d)^{-\chi+1}$). The left-hand side is multiplied with $(1-\rho)$, where $\rho$ is a design parameter to be specified by Chernoff's bound on the probability that the actual number of items in the negative tests is smaller than $(1-\rho)$ times the expected number. By Chernoff's bound~\cite{Chernoff} this is at most $\exp \left (-\rho^2T \left ( \frac{n-d}{n}  \right )^g\right )$. Taking the union bound over these two low-probability events gives us  that Equation (\ref{eq:2}) below holds with probability of error at most $\exp \left( -\rho^2 T \left(\frac{n-d}{n}\right)^g \right) + (n-d)^{-\chi + 1}$.


%The left-hand side of Equation (\ref{eq:1}) refers to the expected number of (possibly repeated) items in negative tests (since there are a total of $T$ tests, each containing $g$ (possibly repeated) items, and the probability of a test being negative equals $((n-d)/n)^g$). The right-hand side of (\ref{eq:1}) refers to the expected stopping-time of the underlying CCP. Setting $g$ to equal $1/ \ln (n/(n-d))$ (a value obtained by optimizing (\ref{eq:1}) w.r.t. $g$) and taking the appropriate limits of $n$ going to infinity and $d$ being much less than $n$ enables us to determine that, in expectation, $T \geq ed \ln n$.

\begin{equation}
\label{eq:2}
(1-\rho)Tg\left ( \frac{n-d}{n} \right )^g \geq \chi (n-d)\ln (n-d)
\end{equation}

So, substituting $g^{\ast} = 1/\ln \left ( \frac{n}{n-d} \right )$ (2), and noting that $\left ( \frac{n-d}{n}\right )^g^{\ast}$ equals $e^{-1}$, we have (\ref{eq:blattyblatt})

%So, substitute $g^{*} = \frac{1}{\ln \left( \frac{n}{n-d} \right)}$ into Equation (\ref{eq:2}), we have

\begin{eqnarray}
	T & \geq & \frac{\chi}{1 - \rho} \frac{(n-d) \ln (n-d)}{g^{*} \left(\frac{n-d}{n}\right)^{g^{*}}} \nonumber \\
	&=& \frac{\chi}{1 - \rho} \frac{(n-d) \ln (n-d)}{\frac{1}{\ln \left(\frac{n}{n-d}\right)} e^{-1}} \nonumber \\
	&=& \frac{\chi}{1 - \rho} \frac{(n-d) \ln (n-d) \ln \left(\frac{n}{n-d}\right)}{ e^{-1}} \nonumber \\
	& \geq & \frac{\chi}{1 - \rho} e \left( d - \frac{d^2}{2(n-d)} \right) \ln (n-d)
\label{eq:blattyblatt} 
\end{eqnarray}


%Differentiate both sides of the equation with respect to $g$, one can obtain the optimal group size 
%$g^*=1 / {\ln \left ( \frac{n}{n-d} \right )}$.
%We derive the coupon collection problem from the perspective of tail estimates. Let $Z_i^r$ be the event that the $i$-th coupon is not picked in the first $r$ trials. Then
%\begin{equation}
%P[Z_i^r]=\left ( 1-1/n \right )^r\leq \lim_{n \to \infty }\left ( 1-1/n \right )^r=e^{-\frac{r}{n}} 
%\end{equation}
%For $r=\beta n \ln n$, we have $P[Z_i^r]\leq n^{-\beta}$. Thus by taking union bound, the tail estimate of coupon collection is achieved as follow.
%\begin{equation}
%P[T>\beta n \ln n]=P[\bigcup_{i}Z_i^{\beta n \ln n}]\leq n\cdot P[Z_i^{\beta n \ln n}]\leq n^{-\beta + 1}
%\end{equation}
%Back to our group testing algorithm, the variance $\error$ of number of tests required around the expectation is
%\begin{equation}
%\error =P\left ( T>\beta \cdot \frac{(n-d)\ln (n-d)}{\left ( \frac{n-d}{n} \right )^gg} \right )\leq (n-d)^{-\beta +1}.
%\end{equation}
%As our focus is the situation when $n$ is very large, we work out the asymptotic lower bound of $T$. In the deduction, we use the estimation of Taylor series for natural logarithm, where $x-\frac{x^2}{2} \leq \log (1+x) \leq x$ for $0 \leq x \leq 1$.

%\begin{eqnarray}
%T({g}^*) & = & \frac{(n-d)\ln(n-d)\ln(\frac{n}{n-d})}{\left ( \frac{n-d}{n} \right )^\frac{1}{\log\left ( \frac{n}{n-d} \right )}}
%\nonumber \\
%& = & \frac{(n-d)\ln(n-d)\ln(1+\frac{d}{n-d})}{\left ( 1-\frac{d}{n} \right )^\frac{1}{\log\left ( 1+\frac{d}{n-d} \right )}}
%\nonumber \\
%& \leq  & \frac{(n-d)\ln(n-d)\frac{d}{n-d}}{\left ( 1-\frac{d}{n} \right )^{\frac{d}{n-d}-\frac{d^2}{2(n-d)^2}}}
%\nonumber \\
%& = & \frac{(n-d)\ln(n-d)\frac{d}{n-d}}{\left ( 1-\frac{d}{n} \right )^{\frac{n\left ( 1-\frac{d}{n} \right )^2}{d\left ( 1-\frac{3d}{2n} \right )}}}
%\nonumber \\
%& \leq & ed\ln n
%\end{eqnarray}

Choosing $\rho = \frac{1}{2}$ and take the error to be

\begin{eqnarray}
		 && e^{-\rho^2 T \left(\frac{n-d}{n}\right)^{g^*}} + (n-d)^{-\chi+1} \nonumber \\
		 &\leq & e^{-\frac{\rho^2 \chi}{1 - \rho}d \ln (n-d)} + (n-d)^{-\chi+1} \nonumber \\
		 &=& (n-d)^{-\frac{1}{2} \chi d} + (n-d)^{-\chi+1} \nonumber \\
		 &\leq & 2(n-d)^{-\chi+1} %\nonumber \\
%		 &=& n^{-\delta} \nonumber
\end{eqnarray}

Taking $2(n-d)^{-\chi+1} = n^{-\delta}$, we have $\chi = \delta \frac{\log n}{\log (n-d)} + \frac{1}{\log (n-d)} + 1$. For large $n$, $\chi = \delta + 1$.

Therefore, the probability of error is at most $n^{-\delta}$, with sufficient large $n$, and the number of test
\begin{equation}
	T \geq 2 (1+\delta) e d \ln n.
\end{equation}

\vspace{0.1in}
